Seele's New Anti-ASIC Consensus Algorithm with Emphasis on Matrix Computation

In this paper, we will present a new PoW consensus algorithm used in Seele's main-net, MPoW (Matrix-Proof-of-Work). Compared to Bitcoin's PoW consensus algorithm, MPoW requires miners to compute the determinants of submatrices from a matrix constructed with n hashes other than brute-force-hashing using a hash function to find the target. This paper will evaluate this algorithm's compatibility with difficulty adjustment. Then we will discuss its efficiency in countering machines with hashrate advantage, and its feasibility to personal computers. We believe more innovative consensus protocols can be developed based on this algorithm.

==> 02_abstract.tex <==
\begin{abstract} 



The blockchain initially gained traction in 2008 as the technology underlying \bitcoin~\cite{bitcoin}, but now has been employed in a diverse range of applications and created a global market worth over \$150B as of 2017. 
What distinguishes blockchains from traditional distributed databases is the ability to operate in a decentralized setting without relying on a trusted third party.  
As such their core technical component is \emph{consensus}: how to reach agreement among a group of nodes. 
This has been extensively studied already in the distributed systems community for closed systems, but its application to open blockchains has revitalized the field and led to a plethora of new designs.

The inherent complexity of consensus protocols and their rapid and dramatic evolution makes it hard to contextualize the design landscape.
%It is crucial to develop a systematic understanding of this area, however, because the scalability and performance of blockchains is becoming a bottleneck to their wide-spread adoption. 
We address this challenge by conducting a systematic and comprehensive study of blockchain consensus protocols. After first discussing key themes in classical consensus protocols, we describe: \first protocols based on proof-of-work (\pow), \second proof-of-X (\pox) protocols that replace \pow with more energy-efficient alternatives, and \third hybrid protocols that are compositions or variations of classical consensus protocols. 
We develop a framework to evaluate their performance, security and design properties, and use it to systematize key themes in the protocol categories described above. This evaluation leads us to identify research gaps and challenges for the community to consider in future research endeavours. \sarahm{Should hint at a few if space.}


\end{abstract}

